Explain by Evidence: An Explainable Memory-based Neural Network for Question Answering

Interpretability and explainability of deep neural networks are challenging due to their scale, complexity, and the agreeable notions on which the explaining process rests. Previous work, in particular, has focused on representing internal components of neural networks through human-friendly visuals and concepts. On the other hand, in real life, when making a decision, human tends to rely on similar situations and/or associations in the past. Hence arguably, a promising approach to make the model transparent is to design it in a way such that the model explicitly connects the current sample with the seen ones, and bases its decision on these samples. Grounded on that principle, we propose in this paper an explainable, evidence-based memory network architecture, which learns to summarize the dataset and extract supporting evidences to make its decision. Our model achieves state-of-the-art performance on two popular question answering datasets (i.e. TrecQA and WikiQA). Via further analysis, we show that this model can reliably trace the errors it has made in the validation step to the training instances that might have caused these errors. We believe that this error-tracing capability provides significant benefit in improving dataset quality in many applications.

==> ack.tex <==
This is Acknowledgements.

==> bg.tex <==
Answer selection is an active area of research with applications in many areas \cite{Wang2015FAQbasedQA,Nakov2015SemEval2015T3,lai-etal-2018-simple,ravichander-etal-2019-question}. Over the past decade, researchers have proposed many deep learning approaches for the task \cite{tay2018hyperbolic,tayyar-madabushi-etal-2018-integrating,lai-etal-2018-review,rao-etal-2019-bridging}. Most early works adopted the Siamese architecture, where the same encoder (e.g., a CNN or a RNN) is used to to create question and answer representations \cite{Yu2014DeepLF,Tan2015LSTMbasedDL,Severyn2015,he-etal-2015-multi}. Typically, there is no explicit interaction between the input sentences during the encoding process. Recently, neural networks based on the Compare-Aggregate architecture have also been extensively studied and evaluated \cite{Wang2017BilateralMM,Bian2017ACM,Shen2017InterWeightedAN,Tran2018TheCA,Tay2018MultiCastAN,Yoon2019ACM}. The Compare-Aggregate architectures capture more interactive features between input sentences than the Siamese architectures, therefore typically have better performance. Under the Compare-Aggregate architecture, small units such as words of the input sentences are first \textit{compared and aligned}. These comparison results are then \textit{aggregated} to compute a final score indicating how relevant the candidate is to the question.


As contextual pretrained language models have made significant breakthrough in various natural language processing tasks \cite{radford2018improving,Devlin2018BERTPO,Liu2019RoBERTaAR,Joshi2019SpanBERTIP}, more recent works on answer selection also leverage these powerful pretrained models \cite{kumar-etal-2019-improving,lai2019gated,laskar2020contextualized,garg2019tanda,soldaini2020cascade}. For example, \newcite{laskar2020contextualized} showed that for answer selection task, the integration of pretrained encoder such as ELMo \cite{Peters2018DeepCW} or BERT \cite{Devlin2018BERTPO} outperforms its integration with traditional GloVe word embeddings \cite{Pennington2014GloveGV}. \newcite{garg2019tanda} demonstrated the benefits of carrying out additional pretraining of BERT-derived models on a large scale answer selection dataset, before fine-tuning it on a target task. \newcite{soldaini2020cascade} proposes an efficient approach to adapt transformer-based language models into a cascade of rankers. Each ranker is used to prune a subset of candidates in a batch, thus effectively improving inference throughput. 

